CNN: Single-label to Multi-label

Convolutional Neural Network (CNN) has demonstrated promising performance in single-label image classification tasks. However, how CNN best copes with multi-label images still remains an open problem, mainly due to the complex underlying object layouts and insufficient multi-label training images. In this work, we propose a flexible deep CNN infrastructure, called Hypotheses-CNN-Pooling (HCP), where an arbitrary number of object segment hypotheses are taken as the inputs, then a shared CNN is connected with each hypothesis, and finally the CNN output results from different hypotheses are aggregated with max pooling to produce the ultimate multi-label predictions. Some unique characteristics of this flexible deep CNN infrastructure include: 1) no ground truth bounding box information is required for training; 2) the whole HCP infrastructure is robust to possibly noisy and/or redundant hypotheses; 3) no explicit hypothesis label is required; 4) the shared CNN may be well pre-trained with a large-scale single-label image dataset, e.g. ImageNet; and 5) it may naturally output multi-label prediction results. Experimental results on Pascal VOC2007 and VOC2012 multi-label image datasets well demonstrate the superiority of the proposed HCP infrastructure over other state-of-the-arts. In particular, the mAP reaches 84.2% by HCP only and 90.3% after the fusion with our complementary result in [47] based on hand-crafted features on the VOC2012 dataset, which significantly outperforms the state-of-the-arts with a large margin of more than 7%.

==> README <==
January 10, 2007

Please note that you may choose to use either double column or single column
formatting. You may wish to use single column formatting when submitting your
paper for review, as it leaves more space for reviewer remarks. The double column format 
is ideal when submitting your final publication materials. The IEEE CS formats articles
in two columns, with 9.5pt Palatino font, and a page size of 7.875 X 10.75. 

June 6, 2006

Added an option to switch between peer review and final submission formats 
into bare_jrnl.tex. 


August 13, 2002

This IEEEtran.cls is the official LaTeX class for authors of the
Institute of Electrical and Electronics Engineers (IEEE) transactions
journals and conferences. In addition to being carried on IEEE's site,
IEEEtran.cls may be found at:

http://www.ctan.org/tex-archive/macros/latex/contrib/supported/IEEEtran/

The CTAN site may have additional files related to non-IEEE uses of this
tool.

As of version 1.6, IEEEtran.cls now provides support for conferences and
A4 paper. Users of previous versions should no longer manually alter margins,
paper sizes, page styles, etc. Also, please note that \author is used
slightly differently from that of V1.5, especially for conferences.
\pubid (if used) must now be placed before \maketitle. \cite is now robust
and can be used within captions without a proceeding \protect.

As with previous versions, The itemize, enumerate, and description lists as
well as \appendix(ces) have enhanced controls and work slightly differently
than is done in traditional LaTeX.

Extensive formal documentation is now available. Enjoy! ;) The appendices
of the user manual contain important information on avoiding commonly
made mistakes, compatibility issues and installation instructions.


Best wishes for all your publication endeavors,

Michael Shell
mshell@ece.gatech.edu



********************* Files **********************

README               - This file.

IEEEtran.cls         - The LaTeX class file.

IEEEtran_HOWTO.pdf   - The user manual.

bare_jrnl.tex        - A "bare bones" starter file for journal papers.




**********************************************************************
 Legal Notice:
 This code and advice is offered as-is without any warranty either
 expressed or implied; without even the implied warranty of
 MERCHANTABILITY or FITNESS FOR A PARTICULAR PURPOSE!
 User assumes all risk.
 In no event shall IEEE or any contributor to this code
 be liable for any damages or losses, including, but not limited to,
 incidental, consequential, or any other damages, resulting from the
 use or misuse of any information contained here.
 
 All statements made here are the opinions of their respective
 authors and are not necessarily endorsed by the IEEE.

 This code/text is distributed under the Perl Artistic License 
 ( http://language.perl.com/misc/Artistic.html ) 
 and may be freely used, distributed and modified.
 Retain all contribution notices and credits.
**********************************************************************



